Bench-CoE: a Framework for Collaboration of Experts from Benchmark

Large Language Models (LLMs) are key technologies driving intelligent systems to handle multiple tasks. To meet the demands of various tasks, an increasing number of LLMs-driven experts with diverse capabilities have been developed, accompanied by corresponding benchmarks to evaluate their performance. This paper proposes the Bench-CoE framework, which enables Collaboration of Experts (CoE) by effectively leveraging benchmark evaluations to achieve optimal performance across various tasks. Bench-CoE includes a set of expert models, a router for assigning tasks to corresponding experts, and a benchmark dataset for training the router. Moreover, we formulate Query-Level and Subject-Level approaches based on our framework, and analyze the merits and drawbacks of these two approaches. Finally, we conduct a series of experiments with vary data distributions on both language and multimodal tasks to validate that our proposed Bench-CoE outperforms any single model in terms of overall performance. We hope this method serves as a baseline for further research in this area. The code is available at \url{https://github.com/ZhangXJ199/Bench-CoE}.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/experiments_copy.tex <==
\section{Experiments}
\label{sec:experiments}


We conducted extensive experiments on both language and multimodal tasks to validate the effectiveness of our proposed method. The experiments aimed to evaluate the performance of our composite model (CoE) compared to individual LLMs under various settings, demonstrating the versatility and robustness of our approach.

% \begin{table}[h]
% \centering
% \begin{tabular}{lcc}
% \hline
% Datasets & Has train subset & Has subject label\\
% \hline
% MMLU Pro & No & Yes\\
% Hellaswag & Yes & No\\
% Winogrande & Yes & No\\
% Big Bench Hard & No & No\\
% \hline
% \end{tabular}
% \caption{Datasets Analyze}
% \label{tab: Datasets Analyze}
% \end{table}

\begin{table}[h]
\centering
\begin{tabular}{lcc}
\hline
Dataset & Training Subset & Subject Labels \\
\hline
MMLU Pro         & No                           & Yes \\
Hellaswag        & Yes                          & No  \\
Winogrande       & Yes                          & No  \\
Big Bench Hard   & No                           & No  \\
\hline
\end{tabular}
\caption{Analysis of Datasets Characteristics}
\label{tab:datasets_analysis}
\end{table}


% 4.1. Language Tasks
\subsection{Language Tasks}

To assess the performance of our method in different scenarios, we performed three sets of experiments on language tasks.

\textbf{Experiment 1: Naive Test}

In this experiment, we trained the router and evaluated the models on the same subset of the benchmark dataset MMLU-Pro\cite{mmlupro}. This setup tests the ability of the router to select the best model when both training and testing data distributions are identical. The test set of MMLU-Pro, consisting of diverse language understanding tasks, was used. We compared five individual LLMs and our composite model (CoE) using both subdomain-level and problem-level routers. The performance of each model is presented in \Cref{tab: Performance on MMLU-Pro test set}.

% ```latex
% Table 1. Performance on MMLU-Pro test set
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
Gemma-2-9b-it\cite{gemma} & 0.5204 \\
Glm-4-9B\cite{glm} & 0.4760 \\
Llama-3-Smaug-8B\cite{llama3-smaug} & 0.3810 \\
Mathstral-7B-v0.1\cite{mistral} & 0.4178 \\
Qwen2-7B-Instruct\cite{qwen2} & 0.4707 \\
\textbf{CoE (Subject-Level Router)} & 0.5235 \\
\textbf{CoE (Query-Level Router)} & \textbf{0.7197} \\
\hline
\end{tabular}
\caption{Performance on MMLU-Pro test set.}
\label{tab: Performance on MMLU-Pro test set}
\end{table}


The CoE with the problem-level router achieved a performance of 0.7197, significantly outperforming all individual models. The CoE with the subdomain-level router also surpassed individual models, though with a smaller margin. This demonstrates that our method effectively leverages the strengths of different models when the data distribution is consistent. The problem-level router's finer-grained control allows it to select the best model for each specific input, leading to substantial performance gains, while the subdomain-level router improves performance by routing inputs to models generally better in specific subdomains.

\textbf{Experiment 2: In-distribution Test}

This experiment evaluates the router's performance when trained and tested on different splits of the same dataset, specifically Winogrande. The router was trained on the Winogrande training set and evaluated on the validation set. We compared four individual LLMs and our CoE with the problem-level router. The results are shown in \Cref{tab: Performance on Winogrande validation set}.


% Table 2. Performance on Winogrande validation set
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
Qwen2-7B-Instruct & 0.6527 \\
Gemma-2-9b-it & 0.6614 \\
Mathstral-7B-v0.1 & 0.5595 \\
Llama-3-Smaug-8B & 0.5706 \\
\textbf{CoE (Query-Level Router)} & \textbf{0.6701} \\
\hline
\end{tabular}
\caption{Performance on Winogrande validation set.}
\label{tab: Performance on Winogrande validation set}
\end{table}


The CoE achieved the highest performance of 0.6701, outperforming all individual models. The improvement over the best individual model (Gemma-2-9b-it) is modest but consistent. Even when the router is trained and tested on different splits, it successfully generalizes and routes inputs to the most suitable models. The problem-level router's ability to adapt to individual inputs contributes to the performance gain.

Additionally, we conducted a similar experiment on the HellaSwag\cite{hellaswag} benchmark. The results are as follows:


% Table 3. Performance on HellaSwag validation set
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
Qwen2-7B-Instruct & 0.7836 \\
Gemma-2-9b-it & 0.8556 \\
Mathstral-7B-v0.1 & 0.6240 \\
Llama-3-Smaug-8B & 0.6304 \\
\textbf{CoE (Query-Level Router)} & \textbf{0.8557} \\
\hline
\end{tabular}
\caption{Performance on HellaSwag validation set.}
\label{tab: Performance on HellaSwag validation set}
\end{table}


The CoE matches the performance of the best individual model (Gemma-2-9b-it), with a slight improvement. This suggests that our method can effectively combine models to achieve or surpass the best single-model performance.

\textbf{Experiment 3: Out-of-distribution Test}

To test the generalization ability of our router, we trained it on one dataset and evaluated it on another. The router was trained on the MMLU-Pro test set and evaluated on the Big-Bench-Hard\cite{bbh} validation set. We compared four individual LLMs and our CoE with both subdomain-level and problem-level routers. The performance is summarized in \Cref{tab: Performance on Big-Bench-Hard validation set}.


% Table 4. Performance on Big-Bench-Hard validation set
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
Qwen2-7B-Instruct & 0.5944 \\
Gemma-2-9b-it & 0.6510 \\
Mathstral-7B-v0.1 & 0.6635 \\
Llama-3-Smaug-8B & 0.6362 \\
\textbf{CoE (Subject-Level Router)} & \textbf{0.6991} \\
\textbf{CoE (Query-Level Router)} & 0.6707 \\
\hline
\end{tabular}
\caption{Performance on Big-Bench-Hard validation set.}
\label{tab: Performance on Big-Bench-Hard validation set}
\end{table}


The CoE with the subdomain-level router achieved the highest performance of 0.6991, outperforming all individual models. The problem-level router also improved over individual models but performed slightly worse than the subdomain-level router in this cross-dataset scenario. The subdomain-level router generalizes better across different datasets because it relies on broader subdomain characteristics rather than specific input features, which may vary between datasets. The problem-level router may overfit to the training dataset's specific input patterns, leading to slightly reduced performance on unseen data.

\textbf{Overall Observations for Language Tasks}

Our method consistently outperforms individual models across different experimental setups. The choice between subdomain-level and problem-level routers depends on the scenario: problem-level routers excel when data distributions are similar, while subdomain-level routers generalize better across different datasets.

% 4.2. Multimodal Tasks
\subsection{Multimodal Tasks}
We extended our experiments to multimodal tasks to demonstrate the versatility of our method.

\textbf{Experiment 1: Naive Test}

In this experiment, we trained the router and evaluated the models on the same subset of the multimodal benchmark dataset MMMU\cite{mmmu} validation set. We compared three individual multimodal LLMs and our CoE with a subdomain-level router. The results are presented in \Cref{tab: Performance on MMMU validation set}.


% Table 5. Performance on MMMU validation set
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
MiniCPM-V-2.6 \cite{minicpm} & 0.4522 \\
InternVL2-8B \cite{internvl, internvl2} & 0.4767 \\
LLaVA-OV-7B \cite{LLaVA-OV} & 0.4667 \\
\textbf{CoE (Subject-Level Router)} & \textbf{0.5178} \\
\hline
\end{tabular}
\caption{Performance on MMMU validation set.}
\label{tab: Performance on MMMU validation set}
\end{table}


The CoE achieved a performance of 0.5178, significantly higher than all individual models. This demonstrates the effectiveness of our method in multimodal settings, effectively combining the strengths of different models.

\textbf{Experiment 2: In-distribution Test}

In this experiment, we trained the router on the MMMU test set and evaluated it on the validation set. The consistent performance across different splits validates the generalization capability of our method. The results are shown in \Cref{tab: Performance on MMMU validation set (trained on test set)}.


% Table 6. Performance on MMMU validation set (trained on test set)
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
MiniCPM-V-2.6 & 0.4522 \\
InternVL2-8B & 0.4767 \\
LLaVA-OV-7B & 0.4667 \\
\textbf{CoE (Subject-Level Router)} & \textbf{0.5078} \\
\hline
\end{tabular}
\caption{Performance on MMMU validation set (trained on test set).}
\label{tab: Performance on MMMU validation set (trained on test set)}
\end{table}


The CoE continues to outperform individual models, achieving 0.5078. The minimal performance drop compared to Experiment 1 indicates good generalization, even when the router is trained and tested on different splits.

\textbf{Experiment 3: Out-of-distribution Test}

To further assess the generalization ability, we trained the router on the MMMU validation set and evaluated it on a different dataset, the MMStar\cite{mmstar} dataset. The results are in \Cref{tab: Performance on MMStar}.


% Table 7. Performance on MMStar
\begin{table}[h]
\centering
\begin{tabular}{ll}
\hline
Model & Performance \\
\hline
MiniCPM-V-2.6 & 0.5433 \\
InternVL2-8B & 0.5922 \\
LLaVA-OV-7B & 0.5586 \\
\textbf{CoE (Query-Level Router)} & 0.5600 \\
\textbf{CoE (Subject-Level Router)} & \textbf{0.6009} \\
\hline
\end{tabular}
\caption{Performance on MMStar.}
\label{tab: Performance on MMStar}
\end{table}


The CoE with subdomain-level router achieved the highest performance of 0.6009, surpassing the best individual model(InternVL2-8B). This confirms that our method generalizes well to different datasets in multimodal tasks, effectively leveraging the strengths of individual models. However, the performance of the CoE with problem-level router has not surpassed that of the best model, which we attribute to the router relying solely on text input for classification, but many text inputs in the multimodal dataset are similar, and distinguishing problem types requires image-based cues. Consequently, the generalization performance of COE with the Problem-Level Router is suboptimal. Therefore, conducting experiments with a multimodal router will be one of our future directions.

\textbf{Overall Observations for Multimodal Tasks}

Our method effectively combines multimodal models to improve performance. The consistent performance gains across experiments validate the flexibility and robustness of our approach in handling different data modalities.

% \textbf{Discussion}
\subsection{Discussion}

\textbf{Advantages of Our Method}

Our composite model consistently outperforms individual models across various tasks and datasets. The method is flexible, working effectively for both language and multimodal tasks, and does not require extensive training or hard-to-obtain labels. By using benchmark performance to generate routing labels, we efficiently leverage the strengths of different models without significant additional resource requirements.

\textbf{Reasons for Performance Gains}

- Leveraging Model Strengths: Different models excel in different subdomains or on specific inputs. Our method capitalizes on these strengths by effectively routing each input to the most suitable model.

- Effective Routing: The router successfully predicts the best model for each input or subdomain, enhancing overall performance.

- Generalization Ability: Especially with subdomain-level routers, the method generalizes well to unseen data distributions, maintaining performance across different datasets.

\textbf{Comparison of Routers}

- Problem-Level Router: Provides fine-grained routing decisions, leading to higher performance when training and testing data are similar. However, it may overfit to the training data, reducing generalization across datasets.

- Subdomain-Level Router: Offers better generalization across different datasets by focusing on broader subdomain characteristics. It may not capture the nuances of individual inputs as effectively as the problem-level router but demonstrates robustness in cross-dataset scenarios.

\textbf{Support for Our Proposed Method}

The experimental results strongly support our proposed method, demonstrating that combining multiple LLMs via an effective routing mechanism leads to superior performance. The method is practical and efficient, as it does not require extensive additional resources beyond what is needed to evaluate individual models.

\textbf{Limitations and Future Work}

While our method shows significant promise, there are areas for improvement:

- Router Complexity: Exploring more sophisticated routing models may further enhance performance, especially in scenarios where the problem-level router overfits.

- Scalability: Assessing the method's scalability with a larger number of models or on larger datasets would be valuable for real-world applications.

- Dynamic Model Integration: Investigating how to dynamically add new models into the composite system without retraining the router from scratch could improve the method's adaptability.



% \textbf{Conclusion}
\section{Conclusion}

Our experiments validate that the proposed pipeline effectively combines multiple LLMs to achieve superior performance across various tasks and datasets. The method leverages the strengths of individual models without the need for extensive training or complex labels, providing a solid foundation for future research in model combination and routing strategies.








%\newpage















%\subsection{CoE Models for Text Processing}

%To validate the effectiveness of the CoE models based on subject classification and their fine-grained counterparts, we conducted comprehensive tests using four datasets: MMLU Pro, Big Bench Hard, Winogrande, and HellaSwag. We compared the results of these models against their respective submodels across multiple metrics.
%This section explores the feasibility and performance enhancements of two types of CoE models, highlighting their superior accuracy rates compared to their submodels through systematic testing.

%\subsubsection{Feasibility Test}

%Initially, we conducted feasibility tests for the designed CoE models on the MMLU Pro dataset. As shown in \Cref{tab: subject CoE and fine-grained CoE on MMLU-PRO}, both the subject classification-based and the fine-grained CoE models exhibited notable improvements in average accuracy over their submodels, with the fine-grained CoE model showing the largest gains.

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lcc@{}}
%    \toprule
%    Model & Average \\
%    \midrule
%    Gemma-2-9b-it & 0.5204\\
%    Glm-4-9B & 0.4760\\
%    Llama-3-Smaug-8B & 0.3810\\
%    Mathstral-7B-v0.1 & 0.4178\\
%    Qwen2-7B-Instruct & 0.4707\\
%    \textbf{CoE(subjects)} & 0.5235\\
%    \textbf{CoE(fine\_grained)} & \textbf{0.7197}\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of subject and fine-grained CoE on MMLU-PRO.}
%  \label{tab: subject CoE and fine-grained CoE on MMLU-PRO}
%\end{table}

% \begin{table*}
%   \centering
%   \begin{tabular}{@{}lccccccccccccccc@{}}
%     \toprule
%     Model & Biology & Business & Chemistry & Computer Science & Economics & Engineering & Health & History & Law & Math & Other & Philosophy & Physics & Psychology & Average \\
%     \midrule
%     % Gemma-2-9b-it & 0.7657 & 0.5311 & & & & & & & & & & & & & \\
%     \bottomrule
%   \end{tabular}
%   \caption{Results. Ours is better.}
%   \label{tab:example}
% \end{table*}


%\subsubsection{Intra-Dataset Generalization Test}

%To further assess the generalization of the fine-grained CoE model, we trained this model on the training sets of the Winogrande and HellaSwag datasets and evaluated its performance on their respective validation/test sets. The outcomes, detailed in \Cref{tab: fine-grained CoE on Winogrande} and \Cref{tab: fine-grained CoE on Hellaswag}, reveal that the fine-grained CoE model consistently outperformed the submodels in validation scenarios.


%\begin{table}
%  \centering
%  \begin{tabular}{@{}lccc@{}}
%    \toprule
%    Model & Train\_m & Validation \\
%    \midrule
%    Qwen2-7B-Instruct & 0.7385 & 0.6527\\
%    Gemma-2-9b-it & 0.7345 & 0.6614\\
%    Mathstral-7B-v0.1 & 0.5941 & 0.5595\\
%    Llama-3-Smaug-8B & 0.6172 & 0.5706\\
%    \textbf{CoE(fine\_grained)} & \- & \textbf{0.6701}\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of fine-grained CoE on Winogrande.}
%  \label{tab: fine-grained CoE on Winogrande}
%\end{table}

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lccc@{}}
%    \toprule
%    Model & Train & Validation \\
%    \midrule
%    Qwen2-7B-Instruct & 0.7862 & 0.7836\\
%    Gemma-2-9b-it & 0.8509 & 0.8556\\
%    Mathstral-7B-v0.1 & 0.6224 & 0.6240\\
%    Llama-3-Smaug-8B & 0.6419 & 0.6304\\
%    \textbf{CoE(fine\_grained)} & \- & \textbf{0.8557}\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of fine-grained CoE on Hellaswag.}
%  \label{tab: fine-grained CoE on Hellaswag}
%\end{table}


%\subsubsection{Cross-Dataset Generalization Test}

%Lastly, to establish the cross-dataset generalization capabilities of our CoE models, we trained the subject-specific and fine-grained CoE models on the MMLU Pro dataset and tested them on the Big Bench Hard dataset. The results, illustrated in \Cref{tab: subject CoE on Big Bench Hard} and \Cref{tab: fine-grained CoE on Big Bench Hard}, demonstrate significant performance enhancements over the submodels, affirming the robustness of both CoE model designs.

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lcc@{}}
%    \toprule
%    Model & BBH validation \\
%    \midrule
%    Qwen2-7B-Instruct & 0.5944 \\
%    Gemma-2-9b-it & 0.6510 \\
%    Mathstral-7B-v0.1 & 0.6635 \\
%    Llama-3-Smaug-8B & 0.6362\\
%    \textbf{CoE(subjects)} & \textbf{0.6991}\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of subject CoE on Big Bench Hard.}
%  \label{tab: subject CoE on Big Bench Hard}
%\end{table}

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lcc@{}}
%    \toprule
%    Model & BBH validation \\
%    \midrule
%    Qwen2-7B-Instruct & 0.5944\\
%    Gemma-2-9b-it & 0.6511\\
%    Mathstral-7B-v0.1 & 0.6635\\
%    Llama-3-Smaug-8B & 0.6362\\
%%    \textbf{CoE(fine\_grained)} & \textbf{0.6707}\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of fine-grained CoE on Big Bench Hard.}
%  \label{tab: fine-grained CoE on Big Bench Hard}
%\end{table}


%\subsection{CoE Models for Multimodal}

%We selected three multimodal models with similar sizes (MiniCPM-V-2\_6, InternVL2-8B, LLaVA-OneVision-7B) as a composite model. Additionally, noting that the MMMU dataset can be divided into 30 disciplines covering areas like science and humanities, we chose it as the training dataset for routing. Through a three-step experiment, we verified that as long as the composite models demonstrate performance diversity on the dataset, our COE model can achieve performance improvement through our routing mechanism.

%\subsubsection{the training routing dataset is the same as the testing routing dataset}

%We trained the router using the validation set of MMMU and tested the performance of the COE model on the MMMU validation set. As shown in the figure, it is clear that as long as the router’s classification is relatively accurate, the COE model, combined in this manner, can at least match the performance of the best model across each discipline. This allows the composite model to leverage each component’s strengths, resulting in performance improvement for the COE model.

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lccc@{}}
%    \toprule
%    Model & Route trained by MMMU val \\
%    \midrule
%    MiniCPM-V & 0.4522\\
%    InternVL2-8B & 0.4767\\
%    LLaVA-OV & 0.4667\\
%    \textbf{CoE} & \textbf{0.5178}\\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of CoE on MMMU val.}
%  \label{tab: CoE on MMMU val}
%\end{table}

%\subsubsection{the training routing dataset and the testing routing dataset are different, but have the same distribution}

%We trained the router using the test set of MMMU and evaluated the COE model’s performance on the MMMU validation set. As shown in the figure, since the data distribution of the MMMU test set is the same as that of the validation set, the router can accurately classify the validation data into 30 subjects. Consequently, the COE model performs as well as, or even surpasses, the best individual model across most subjects.

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lccc@{}}
%    \toprule
%    Model & Route trained by MMMU test \\
%    \midrule
%    MiniCPM-V & 0.4522 \\
%    InternVL2-8B & 0.4767 \\
%    LLaVA-OV & 0.4667 \\
%    \textbf{CoE} & \textbf{0.5078} \\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of CoE on MMMU test.}
%  \label{tab: CoE on MMMU test}
%\end{table}

%\subsubsection{the training routing dataset and the testing routing dataset are completely different}

%After training the router on the MMMU test set, we tested the performance of the COE model on other multimodal benchmarks to verify the generalization of this paradigm. We observed that the MMstar dataset can be categorized by class, and that the three selected models in the combination exhibit diverse performance across it. Although the data distribution of the MMMU dataset may differ significantly from that of the MMstar dataset, and MMstar does not fully cover the 30 disciplines, as shown in the figure, the COE model still achieves performance improvement.

%\begin{table}
%  \centering
%  \begin{tabular}{@{}lccc@{}}
%    \toprule
%    Model & Route trained by test MMMU test \\
%    \midrule
%    MiniCPM-V & 0.5433 \\
%    InternVL2-8B & 0.5922 \\
%    LLaVA-OV & 0.5586 \\
%    \textbf{CoE} & \textbf{0.5982} \\
%    \bottomrule
%  \end{tabular}
%  \caption{Results of CoE on MMstar.}
%  \label{tab: CoE on MMstar}
%\end{table}
